The power of indirect social ties

While direct social ties have been intensely studied in the context of computer-mediated social networks, indirect ties (e.g., friends of friends) have seen little attention. Yet in real life, we often rely on friends of our friends for recommendations (of good doctors, good schools, or good babysitters), for introduction to a new job opportunity, and for many other occasional needs. In this work we attempt to 1) quantify the strength of indirect social ties, 2) validate it, and 3) empirically demonstrate its usefulness for distributed applications on two examples. We quantify social strength of indirect ties using a(ny) measure of the strength of the direct ties that connect two people and the intuition provided by the sociology literature. We validate the proposed metric experimentally by comparing correlations with other direct social tie evaluators. We show via data-driven experiments that the proposed metric for social strength can be used successfully for social applications. Specifically, we show that it alleviates known problems in friend-to-friend storage systems by addressing two previously documented shortcomings: reduced set of storage candidates and data availability correlations. We also show that it can be used for predicting the effects of a social diffusion with an accuracy of up to 93.5%.

==> sections/correlations.tex <==
%=================================================
\section{Examine All Kinds of Correlations}
%=================================================
In this section, we investigate all kinds of correlations among original edge weights, jaccard coefficient and social strength value with the three datasets---CA-I, CA-II and TF2.

\subsection{Methodology}
Notably, original edge weights and jaccard coefficient values are the value of two directly connected nodes in the graph while social strength is calculated when two nodes are not directly connected.
In order to obtain correlations in the same condition (i.e., the same pair of nodes), two strategies are used:
\begin{itemize}
	\item The social strength of directly connected edge is equal to the edge weight after normalization.
	\item First remove the directly connected edge (e.g., edge AB), then calculate social strength of AB. 
\end{itemize}
In the second method, because of the edge remove, some pair of nodes' social strength values decrease to zero (isolated or not in the path length).
We consider these two scenarios (with and without zero social strength values) separately.
Therefore, the results of second method are divided into two cases: social strength values include zeros and nonzero social strength values.
The results are presented in Table~\ref{tab:correlation2} and Table~\ref{tab:correlation3}.

\subsection{Results}
The results of the first method are shown in Table~\ref{tab:correlation1}.
\begin{table} 
\begin{center}
\itshape  
\begin{tabular}{|l||c|c|c|}
\hline
Networks &Cor(edge\_weight, jaccard) & Cor(edge\_weight, ss) & Cor(jaccard, ss)\\
 \hline\hline 
 CA-I & {\itshape 0.154}& 0.263 & -0.156 \\ 
 \hline
 CA-II & {\itshape 0.198}  & 0.288 & -0.035\\ 
\hline 
TF2 & {\itshape 0.098}  &  -0.043 & -0.123\\ 
\hline 
\end{tabular}  
\end{center}
\caption{The statistics of Pearson correlation coefficient among edge weights, Jaccard coefficient and the Social Strength values.}\label{tab:correlation1}
 \end{table}
 
 
\begin{table} 
\begin{center}
\itshape  
\begin{tabular}{|l||c|c|c|}
\hline
Networks &Cor(edge\_weight, jaccard) & Cor(edge\_weight, ss) & Cor(jaccard, ss)\\
 \hline\hline 
 CA-I & {\itshape 0.154}& 0.241 & 0.618 \\ 
 \hline
 CA-II & {\itshape 0.198}  & 0.397 & 0.585\\ 
\hline 
TF2 & {\itshape 0.098}  &  0.272 & 0.481\\ 
\hline 
\end{tabular}  
\end{center}
\caption{The statistics of Pearson correlation coefficient among edge weights, Jaccard coefficient and the Social Strength values that are calculated by removing directly connected edges.}\label{tab:correlation2}
 \end{table}
 
 
\begin{table} 
\begin{center}
\itshape  
\begin{tabular}{|l||c|c|c|c|}
\hline
Networks &Cor(edge\_weight, jaccard) & Cor(edge\_weight, ss) & Cor(jaccard, ss) & Per. of Removed Zeros\\
 \hline\hline 
 CA-I & {\itshape 0.09}& 0.217 & 0.342 & 36.6\%\\ 
 \hline
 CA-II & {\itshape 0.184}  & 0.398 & 0.528 & 9.3\% \\ 
\hline 
TF2 & {\itshape 0.046}  &  0.240 & 0.395 & 18.1\%\\ 
\hline 
\end{tabular}  
\end{center}
\caption{The statistics of Pearson correlation coefficient among edge weights, Jaccard coefficient and the Social Strength values that are calculated by removing directly connected edges and removed edges with zero social strength values.}\label{tab:correlation3}
 \end{table}
 
 
{\textcolor{red}{Identification du Systme}}




==> sections/diffusion.tex <==
%\section{Experiments}
\section{Leveraging Social Strength  to Predict Information Diffusion Paths on OSNs}
The goal of this experiment is to show that Social Strength (SS) can predict information spreading paths in OSNs.
Notably, the predicted diffusion paths are beyond 1-hop relationships, for example 2-hop away paths. I.e., if we know a node has some information and would like to disseminate it at timestamp $t_0$, we can predict what other nodes will accept the disseminated information at timestamp $t_2$ instead of only timestamp $t_1$.

If we could predict the diffusion paths ahead, we can watch those dangerous nodes who might accept rumors or diseases in the near future.
In our experiments, currently, we only focus on predicting diffusion paths at 2-hop distance with single seed source.

\subsection{Experiment Design}
This section describes the experiments of applying social strength metrics on information diffusion paths prediction and the prediction performance.


\subsubsection{Experimental Setups}
%{\bf Implementation.} 
{\bf Step 1(Diffusion Simulation):} To obtain the information about which nodes accepted the passed on information at different timestamps (ground truths) on a OSN's information diffusion processes, we employed a widely used Susceptible-Infected (SI)~\cite{} model to simulate diffusion processes and recorded all the diffusion paths and timestamps information, namely, in each timestamp which nodes accepted the passed on information from its neighbors (not all neighbors but those already accepted the information in the previous phases).
As~\cite{} describes, SI model is a probability-based diffusion model and only has two phases, either accepted the information or not.
There must be some seeds (information source holders) in the beginning timestamp ($t_0$) to initiate the diffusion.
Thus, we randomly selecting seeds in the cold-start phase.
For simplicity, we set the spreading probability from an infected node $v_i$ to its nearest susceptible neighbor $v_j$ was made proportional to the edge weight $w_{i,j}$.
Introducing a constant of proportionality x, the time independent probability of passing information from $v_i$ to $v_j$ can be written as $P_{i,j}$ = x$w_{ij}$, where increasing x results in a higher spreading probability.
The most obvious choice is to set x = 1/$max(w_{ij})$ (proportional to the global maximum edge weight in the graph), in which case for the globally strongest link $P_{i,j}$ = 1 and for all others $P_{i,j}$ is smaller than 1.
We set a threshold T, which is in the range between the $P_{min}$ and the maximum $P_{max}$.
Here, $P_{min}$ is the minimum probability that when the threshold T $\leq T$ the information will disseminate to all the nodes in the graph.
Likewise, if the threshold T $\geq P_{max}$, almost no node will accept the information.
For more general scenarios, if $P_{ij}$ $\geq T$, information will spread through the $E_{ij}$, vice versa.

{\bf Step 2 (Predict diffusion paths by using social strength values):} We calculate social strength values between the seed and its 2-hop neighbors, then convert the social strength values to social ranks, i.e., allocate a rank a node's 2-hop neighbors in terms of social strength values. 
Because of the asymmetric characteristic of social strength metrics (section...), the according social ranks are also asymmetric. 
For example, a pair of nodes A and B, the social rank of B from A's perspective is 1 while the social rank of A from B could be 3. 
Such asymmetric social ranks are consistent with real-world social relationships among people, which can better estimate people's social ties compared to symmetric ties.

After obtaining the social ties, we need a cut-off point to decide whether a node's 2-hop neighbors will accept the information from it in $t_2$ or not.
The standard we use for the cut-off threshold is both social ties of a pair of users should be high ($rank_{AB}$ and $rank_{BA}$ both are among the top 10\% social ranks in each rank list).
Then, the cut-off threshold can classify a node's all 2-hop neighbors into two categories: information-accepted nodes and information-denied nodes.

In our experiments, we focus paths prediction on single seed and 2-hop distance, which means information sources are controlled by a single node in the cold-start phase and with the node information in $t_0$, we predict the possible nodes that will accept the spreading information in $t_0$ instead of $t_1$.
This 2-hop long timestamp paths prediction can supply more time spaces for people or decision makers to take actions to contain rumor disseminations or choose users who are influential in information spreading for advertisement delivers.
Notably, multiple seeds diffusion and farther distance paths can be predicted by extending from 2 hops. 

{\bf Step 3: (Prediction evaluation):} Compare the prediction results with the ground truths we obtained in Step 1, we can use widely-used evaluation metrics to evaluation the performance of social strength metrics on information diffusion paths predictions.

\subsubsection{Results and Evaluation}
{\bf Dataset.} We used the three OSNs datasets (CA-I, CA-II and TF2) as described in the previous section and all the experiments results are average values of 100 iterations.
The input of the simulation must be a weighted graph where edge weights illustrate the social ties between two directly connected nodes (or users).
The prediction results of CA-I are shown in Figure~\ref{fig:prediction-evaluation-small} and Figure~\ref{fig:prediction-evaluation-big}, and we can see that almost all the sensitivities are above 0.65 and the accuracies and specificities are over 0.6 when the threshold varies from 0.01 to 0.10.
The range we chose for the threshold is based on the edge probability distribution, for example, in CA-I network, 0.01 is the boundary for disseminating information throughout the entire graph and 0.10 is the boundary of no node accepts any information in the network. 
Similarly, we choose 0.007 and 0.07 as the two boundaries of CA-II.
Thus, the threshold between these boundaries represent the majority of diffusion cases.

{\bf Baseline:} In order to better show that social strength has positive effect on predicting diffusion paths, we compare the prediction results with a baseline results.
Here, the baseline is defined as assume all 2-hop friends accept the spreading information in $t_2$.
The comparison results are shown in Figure~\ref{fig:small-baseline} and Figure~\ref{fig:big-baseline}, where social strengths show better performance than the baseline results.

%in Figure~\ref{fig:prediction-evaluation} with a baseline. 

However, we also found that our prediction results highly depend on the cut-off thresholds meanwhile the thresholds. 
If we change the thresholds the prediction results will change. 

\begin{figure}[tbhp]
\begin{center}
      \graphicspath{{./figure/}}
      \includegraphics[scale=0.6]{prediction-accuracy-small.pdf}
      \caption{Evaluate prediction results of CA-I by sensitivity, specificity and accuracy.}\label{fig:prediction-evaluation-small}
\end{center}
\end{figure}



\begin{figure}[tbhp]
\begin{center}
      \graphicspath{{./figure/}}
      \includegraphics[scale=0.6]{small-baseline.pdf}
      \caption{Compare social strength prediction results of CA-I with baseline.}\label{fig:small-baseline}
\end{center}
\end{figure}



\begin{figure}[tbhp]
\begin{center}
      \graphicspath{{./figure/}}
      \includegraphics[scale=0.6]{prediction-accuracy-big.pdf}
      \caption{Evaluate prediction results of CA-II by sensitivity, specificity and accuracy.}\label{fig:prediction-evaluation-big}
\end{center}
\end{figure}



\begin{figure}[tbhp]
\begin{center}
      \graphicspath{{./figure/}}
      \includegraphics[scale=0.6]{big-baseline.pdf}
      \caption{Compare social strength prediction results of CA-II with baseline.}\label{fig:big-baseline}
\end{center}
\end{figure}



 




==> sections/social_strength.tex <==
%==============================
\section{Social Strength Metrics Definition}
%==============================
We normalize all the edge weights to help us scale the social strength among different users.
Also, this normalization results in asymmetrical relationships between user i and j. 
The inherent reason is that the normalization is relevant to each user's degree. 
\begin{equation}
%NW(i, j) = \frac{\sum\omega(i, j)}{\max_{\forall j \in J_i} (\sum \omega(i,j))}
NW(i, j) = \frac{\sum_{\forall \lambda \in \Lambda_{i,j}}\omega(i, j, \lambda )}{\sum_{\forall k \in N_i}\sum_{\forall \lambda \in \Lambda_{i,k}} \omega(i,k,\lambda)}
\label{eq:nw}
\end{equation}
Where $\omega(i, j) $ is the edge weight between user $i$ and $j$.
$\Lambda_{i,j}$ is the set of labels (e.g., relationships based on work, sport, and school) of edges connecting from user $i$ to $j$.
Thus, the numerator is the aggregation of all edge weights from user $i$ to $j$ with all different labels.

For denominator, $N_i$ is the set of directly connected neighbors from $i$ to others. 
Denominator sums all edge weights from user i to all other connected users with all labels.

Assuming that $P_{i, m}$ is the set of different paths joining two indirectly connected users $i$ and $m$, and $Node_{path}$ is the set of nodes on the path.
we can quantify the social strength between them from $i$'s perspective over a multi-level n-hop path using this function:
\begin{equation}
\begin{split}
SS(i,m) = 1- \Pi_{\forall path \in P_{i,m}\cap path=n} (1- \\
  \frac{min_{j,...,k\in Node_{path}}\{NW(i,j),...,NW(k,m)\}}{n})
\label{eq:socs}
\end{split}
\end{equation}

Certain type of social strength---for example, labeled as work, sport or school---can be calculated by the following equatios:
\begin{equation}
NW_t(i, j) = \frac{\omega(i, j, \lambda_t )}{\sum_{\forall k \in N_i \cap\lambda=\lambda_t}\sum_{\forall \lambda \in \Lambda_{i,k}} \omega(i,k,\lambda_t)}
\label{eq:nw}
\end{equation}
Where t is any type of relationship between two users.
All other definitions are the same as Equation (1).

\begin{equation}
\begin{split}
SS_t(i,m) = 1- \Pi_{\forall path \in P_{i,m,t}\cap path=n} (1- \\
  \frac{min_{j,...,k\in Node_{path}}\{NW_t(i,j),...,NW_t(k,m)\}}{n})
\label{eq:socs}
\end{split}
\end{equation}
$P_{i, m,t}$ is the set of different paths joining two indirectly connected users $i$ and $m$ with label t, and $Node_{path}$ is the set of nodes on the path.

We define the social strength value between two directly connected users as the results of normalization (calculate with formula 1), and this result is consistent with formula 2 if replace n to 1. 
